Visible Light Communication for Wearable Computing

Visible Light Communication (VLC) is emerging as a means to network computing devices that ameliorates many hurdles of radio-frequency (RF) communications, for example, the limited available spectrum. Enabling VLC in wearable computing, however, is challenging because mobility induces unpredictable drastic changes in light conditions, for example, due to reflective surfaces and obstacles casting shadows. We experimentally demonstrate that such changes are so extreme that no single design of a VLC receiver can provide efficient performance across the board. The diversity found in current wearable devices complicates matters. Based on these observations, we present three different designs of VLC receivers that i) are individually orders of magnitude more efficient than the state-of-the-art in a subset of the possible conditions, and i) can be combined in a single unit that dynamically switches to the best performing receiver based on the light conditions. Our evaluation indicates that dynamic switching incurs minimal overhead, that we can obtain throughput in the order of MBit/s, and at energy costs lower than many RF devices.

==> end.tex <==
\section{Conclusion}
\label{sec:end}

VLC is an enabler for many networked applications, but is challenging 
in mobile settings since mobility induces rapid, drastic and unpredictable 
changes in the SNR. In this paper we present three different designs for
VLC receivers with a performance that is orders of magnitude better than
the existing state-of-the-art for VLC receivers. Our results show that, for example, the
\ulp receiver's energy consumption is lower even than those of RF chips
designed for low power consumption. Also, our \highspeed VLC receiver
achieves a throughput that is orders of magnitudes higher than 
state-of-the-art embedded VLC receivers and on par with WiFi and Bluetooth
chips in both throughput and energy consumption. Nevertheless, the
individual receivers alone cannot cope with the rapid SNR changes
in mobile settings. Towards this end, we design a switching logic that
we implement on an integration unit. Our experiments show that 
our logic is able to rapidly adapt to the fluctuating light conditions and
select the best performing receiver.    
Our work broadens the application area of VLC to mobile settings
by, for example, enabling the transmission of data from a VLC infrastructure
to resource-constrained on-body sensors.

%%% mode: latex
%%% TeX-master: "main"
%%% End: 



==> implementation.tex <==




==> motivation.tex <==
VLC  lacks an accessible functional equivalent of a radio chip. Consequently, the logic to receive and
demodulate VLC transmissions is often executed as an application on the host MCU~\cite{epsilon,retrovlc,ledtoled,wang2015open}. 
This couples the ability to receive transmissions closely to the abilities and constraints of the device. Embedded devices are extremely 
heterogeneous in their capabilities, constraints and requirements. This makes it difficult to have 
a universal design of the receiver. Hence, we first start by identifying major classes of embedded devices and their requirements and constraints on VLC.

\fakepar{Intermittently Powered Devices}  An emerging class of embedded devices comprise of battery-free devices.
These devices operate only on energy harvested from ambient sources like  RF signals~\cite{ambientbackscatter}, 
temperature fluctuations~\cite{tempchange} or light~\cite{retrovlc}.  Consequently, these devices have an extremely stringent
energy budget and are Intermittently Powered (IPD). These devices could benefit from being able to receive 
low data rate control messages using VLC. E.g. synchronisation of these devices is difficult, VLC could help this. On such devices supporting VLC while beneficial is
challenging. 

The fundamental operation to receive VLC transmissions is to keep track of light intensity fluctuations. A photodiode
helps to keeps track. A photodiode in itself needs very little or no power. Its output, however, needs to be
amplified and digitized before it can be used. Both these operations need energy expensive components -
amplifier and analog to digital (ADC) converter. IPD devices have very limited available energy rendering this approach infeasible. This is precisely why there is no 
existing work to communicate with these devices using visible light.  E.g.  One class of IPD devices comprise of the 
Computational RFID (CRFID) platforms like the Moo~\cite{zhang2011moo} and WISP~\cite{WISP}.  These devices 
operate on energy harvested of ambient RF signal. The RF signal itself is generated by a RFID reader. 
On these devices also ADC operations are avoided. E.g. Zhang et al.~\cite{bitbybitbackscatter} explains 
that a single ADC operation consumes as much energy  as transmitting 27 bits on  Moo~\cite{zhang2011moo}.  
 
 %Texas Instruments (TI) MSP430 series of MCU have been used extensively on the CRFID platform.  MSP430 has been getting energy efficient with time. E.g.  MSP430 FR5969~\cite{MSP430FR5969} used on the state-of-the art CRFID platform WISP 5.0~\cite{WISP} 
 %%consumes only 100 $uA$ of current in active mode, as compared to 250 $uA$ by MSP430F2132~\cite{MSP430F2132} used by Moo~\cite{zhang2011moo}.
 
 %In this experiment, we verify if the ADC conversions are still energy expensive on the newer generation of CRFID platforms. We evaluated the cost of ADC operations on WISP 5.0\cite{WISP}. We keep a WISP about 15 cm from the antenna of a software defined radio (SDR). 
 %The SDR generates a carrier signal of 10 dBm strength. The WISP after harvesting sufficient amount of energy, powers on and toggles one of the GPIO pins high. This pin remains high till WISP runs out of energy. We capture this transition using a high-speed logic 
 %analyzer from Saleae\cite{logicanalyzer}. We specifically evaluate the effect of operating clock frequency of the MCU,  and the effect of ADC, and the sampling frequency of the ADC on the node on-time. Figure \ref{wispontime} shows the result of  the experiment. 
%We did 3 iterations of each experiment, collecting samples for 300 seconds. We observe a substantial decrease in the WISP on-time as the ADC is turned on.  Surprisingly, changing the sampling rate of the ADC has a 
%very little effect on the on-time. Also, as expected increasing the MCU clock frequency substantially increases the energy consumption and the node on-time drops significantly. 
%As the demodulation logic runs on the MCU, and a certain number of CPU instructions needs to be executed to receive each bit.  Consequently, the achievable bitrate is a function of the operating clock frequency. The reduced on-time would affect the achievable bitrate.
 

\fakepar{Battery-powered Embedded Devices}  Battery powered devices are the largest class of embedded devices. 
These devices are usually equipped with low powered MCU operating at few $MHz$ to 10s of $MHz$ of clock frequency. 
Conserving energy is one of the important tasks on these devices. This helps to extend the battery lifetime. 
These devices are usually networked using Bluetooth LE/Zigbee making them very prone to CTI~\cite{Liang:2010:SWI:1869983.1870014}.
VLC could prove to be an alternative to mitigate CTI.  There has been, however,  only recent efforts to connect these 
devices using visible light~\cite{ledtoled,hybridvlc,Yang:2015:WAL:2742647.2742648}.  These attempts are very limited. 
E.g. Schmid et al. reports a maximum throughput of 800 b/s at RX power consumption of 288 $mW$~\cite{ledtoled}. This
is orders below in efficiency as compared to RF standards like Zigbee/Bluetooth. To be a viable alternative, on these devices
 the energy/bit for VLC has to be  comparable (if not better) to RF communication.

 One of the primary reasons for this is due to the use of ADC to detect light intensity changes.
 This needs constant sampling of the photodiode using ADC: First to detect a transmission 
 and next to  receive sent bits. The constant polling of the light sensor using ADC keeps the MCU active. 
 ADC by itself is also energy expensive. This increases the energy consumption substantially. 
 In addition, a minimum number of instructions are executed to receive each bit. E.g. to sample photodiode using ADC, 
 check light levels, interpret bits and finally store in buffer. This further reduces the achievable bitrate especially 
 at low operating clock frequencies.

\fakepar{Single Board Computer}  Single Board Computers (SBC) like the Raspberry Pi\cite{RaspberryPi} , BeagleBone\cite{BeagleBone} or Intel Edison\cite{Edison} 
are increasingly becoming popular.  There could be many useful applications to network these devices using VLC. 
E.g. Wang et al. uses one such SBC as a research platform~\cite{wang2015open}.
These are extremely powerful operating at 100s of $MHz$ of operating clock frequency.  They also offer easy access to the GPIO ports, 
interfaces (I2C,SPI,UART) and peripherals including the ADCs. 
This might suggest it might be easy to network these devices using VLC. However, this is not the case. 

One of the primarily limitation arises from using a complex operating system like GNU/Linux on these devices. To keep track of light intensity changes, often a separate process is spawned. This process is  only one of the many running process on this system. Consequently, the operating system  
interleaves its execution. This  affects the achievable data rate and introduces errors.  Furthermore, this process is implemented as part of user space,
while the access to the ADC goes through the kernel space. This further introduces latency and affects the achievable data rate.
E.g. Wang et al. achieves only 18 $kbps$ with the OpenVLC platform built around BeagleBone running GNU/Linux~\cite{wang2015open}. They explain that their
achievable throughput is limited by the operating system even though they can transmit at much higher data rate. Real-Time Linux alleviates some of these issues.  
RT-Linux, however, only supports ADC sampling precisely only up-to certain frequency~\cite{brown2010fast}.





 \fakepar{Other devices} Other devices like network routers, home entertainment systems etc are almost at periphery of computers and embedded devices.
 There could be many use cases to network these using VLC. E.g. In a smart home VLC could be used to control a home entertainment system, or 
 VLC could provide an alternative side-channel to coordinate router transmissions to mitigate interference~\cite{FreeBee}. These applications possibly might
 need only few bytes of control information to be sent using VLC. However, these devices impose new set of constraints making this difficult.
 
 Most of these devices are sold as black box providing little or no access to the lower level hardware or software interfaces providing access only to a USB port.
 This limits the possibility of attaching external light sensor. It is also often non trivial to run custom firmware or modify the operating system significantly. 
 
 In summary,  the different class of embedded devices have very different constraints, requirements and needs in terms of data rate. We list some of  these in the Table~\ref{embeddedtable}.
 All of these could benefit from downlink using VLC. However, this is non trivial to achieve. We address these issues with the design of receiver discussed in Section~\ref{design}.


%\begin{figure}
%\centering
 %\includegraphics[width=0.4\textwidth]{wispontime.pdf}
 %\vspace{-4mm}
  %\caption{ADC conversions are energy expensive.  \capt{ The figure illustrates the effect of sampling the onboard ADC on the operating time of the WISP 5.0 platform. We notice a substantial drop in the time the MCU remains active as the ADC is enabled.  The operating clock frequency also has a significant effect.   } }
  %\label{wispontime}
  % \vspace{-4mm}

%\end{figure}





==> relatedwork1.tex <==
\section{Related Work}
\label{sec:relwork}

This section presents related work.
While there is not yet much related VLC work for wearable devices,
a larger body of work exists in the areas of visible light communication, visible light-based sensing and body area networks. 

\fakepar{VLC for wearable devices} Using VLC to communicate with wearable devices is an emerging area that is only starting to get attention. Zhang et al.\ point out that VLC channels are highly deterministic for given node locations and orientations~\cite{zhang2015dancing}.  They show, however, that small changes in movement or orientation can lead to SNR variations of tens of dB even in very short time durations which makes mobility challenging. To cope with mobility, they design an in-frame rate adaption. Hong and Chen also tackle the challenge of mobility in VLC~\cite{hong2016toward}. They use a pre-coding scheme to recover the original VLC signal showing improved performance compared to conventional OFDM schemes. Our efforts are orthogonal in that we design novel VLC receivers that we integrate to achieve stable VLC performance despite the challenging link dynamics in mobile scenarios.

\fakepar{Visible light communication}  While VLC for wearable devices is an emerging area, significant research efforts have gone into high throughput VLC~\cite{1649137}.
Existing solutions achieve very high throughput, in the order of $GBit/s$~\cite{6701327}. 
For example,  Tsonev et al.\ demonstrate  data rates exceeding 3 $GBit/s$ using OFDM modulation and gallium nitride LEDs~\cite{6701327}.
These efforts are orthogonal to ours as they target different applications.
They intend to replace WiFi and hence optimize for high throughput, using specialised 
photodiodes coupled with high-speed ADC/Oscilloscope to sample optical channels and receive transmissions.
The inherent complexity and high energy consumption make such solutions unsuitable for wearable 
and embedded devices.

VLC systems predominantly use photodiodes as light sensors~\cite{addref}.
Recently,  Wang et al.\ demonstrate the use of a solar panel as a light sensor, coupled to an energy-expensive voltage amplifier~\cite{wang2015design}.
They achieve 11.84 $MBit/s$ using OFDM as a modulation scheme.
Their design, however, is unsuitable for energy harvesting wearable devices. 
As a comparison, the \ulp receiver does not need voltage 
amplifiers and ensures little processing overhead for constrained energy harvesting devices.

Recent efforts to connect embedded devices using VLC achieve much lower throughput.\tv{lower than what? You can also write "achieve low throughput"}
Giustiniano et al.\ de\-monstrate LED to LED communication at a throughput of 800 $bps$~\cite{6402861}.
Tian et al.\ present a VLC system working at light levels imperceptible to human eyes, achieving a throughput of 1.6 ~$kbps$~\cite{darkVLC}. 
Rajagopal et al.\ transmit data to both cameras and embedded devices~\cite{hybridvlc}. One of their use cases is similar to ours, in that it presents a low-power wake-up mechanism for energy-constrained devices. 
Our work is complementary to these systems, in that it tackles the problem of efficient communication to a broad class of diverse embedded devices.
Our VLC receivers achieve both much higher throughput and lower energy consumption even in challenging mobile scenarios.

Li et al.'s Retro-VLC enables full-duplex VLC~\cite{Li:2015:REB:2699343.2699354}.  
The system achieves 10 $KBit/s$ of downlink throughput at an energy cost of \SI{125}{\micro\watt}.
To achieve ultra low power, Li et al.\ use of a thresholding circuit, like we do.
However, while we use a solar cell as light sensor, Retro-VLC employs a photodiode that significantly increases energy consumption.
As a comparison, our \ulp receiver achieves 50 $KBit/s$ with a power consumption of \SI{0.5}{\micro\watt}, which represents a 250x improvement in energy consumption over Retro-VLC.
   
 \fakepar{Visible light-based sensing} Recently, VLC is also applied for sensing applications, such as indoor localization and gesture recognition.
For example, Epsilon~\cite{epsilon} uses fixed LED luminaries to broadcast beacons received by an embedded device leading to submeter accuracy in office environments.
Rajagopal et al.\ present a system that communicates using visible light to mobile receivers and embedded tags to enable room level localization~\cite{Rajagopal:2014:VLL:2602339.2602367}.
Li et al.\ describe a system that uses an array of photodiodes to  track user gestures by detecting the shadow they cast~\cite{Li:2015:HSU:2789168.2790110,practicalhumansensing}. Zhang et al.'s system uses light sensors to track the movement of fingers to achieve  gesture detection~\cite{Okulli} with high accuracy.
Similar to us, these systems use off-the-shelf components together with embedded platforms as receivers. Our work, however, targets mobile devices where the link changes can be significant even during short time spans.

%Differently, however, based on our abstract architecture we can instantiate different VLC receivers optimized for the specific requirements, and show that this approach leads to throughput and energy consumption figures far beyond what these systems achieve.


\fakepar{Networking wearable devices and body area networks} 
Since body area networks can monitor important parameters such as human��s 
health status and motion patterns, they have received a lot of
attention~\cite{chen2011body}. Recent work in the area by 
%Networking wearable devices is an 
%emerging area of research with some recent attempts. 
Hessar et al.\ have presented
a novel mechanism that enables commodity input
devices such as those present on wearable devices to communicate 
securely using body as channel~\cite{hessar2016enabling}.
Zhang et al.\ devise an ultra low power 
mechanism to backscatter and shift ambient wireless
signals to network sensors on 
wearable devices~\cite{zhang2016enabling}. Our efforts are complementary to these existing attempts but we use visible light rather than RF.


==> solarcellexp.tex <==
\fakepar{Solar cell as receiver} 

% motivation and purpose
Small-scale solar cells have not yet been used as a light sensor for VLC communication. Therefore, we first investigate the feasibility of using a solar cell as a light sensor by evaluating a number of solar cells that  differ in size, type and efficiency. We also determine the maximum achievable bitrate in our settings.

% pre-conditions
To be able to receive bits, we must be able to detect changes in the light intensity levels. This requires sufficient difference in amplitudes levels as seen by the solar cell corresponding to the ON and OFF states of the transmitting bulb. Intuitively, we expect that when the transmitting bulb is ON,  the solar cell's amplitude level should be at the maximum, and with
the bulb switched off it should be zero.  Initial experiments show, however, that this is not the case: the solar cell exhibits capacitance which affects its ability to respond quickly to the changing light conditions. Hence, at high bitrates the solar-cell discharges slowly affecting the ability to distinguish between the two states of the bulb.

% setup
We use a setup similar to the one described earlier. \tv{similar is always tricky since reviewers start to wonder about the difference}
We program the transmitting bulb to generate an alternating sequence of $1s$ and $0s$.
We use seven different solar cells with a small form factor but different capabilities from Digikey~\cite{digikey}. These solar cells are:  Slmd600h10l~\cite{SLMD600H10L}, Kxob22-01x8f~\cite{KXOB2201X8F}, Slmd121h04l~\cite{SLMD121H04L}, Slmd121h08~\cite{SLMD121H08}, Slmd121h09l~\cite{SLMD121H09L},  Am1456~\cite{AM1456}  and  Am5610~\cite{AM5610}.  The first five are monocrystalline with different dimensions and parameters, while the last two are amorphous silicon solar cells. We connect all solar cells to the ADC of the logic analyzer to find the peak-to-peak difference $V_{pp}$ in the amplitude of the received signal.

% result
Figure~\ref{solarcellbitrate} demonstrates that all the solar cells exhibit similar behaviour: As the sending bitrate increases, the solar cells' ability to distinguish between the two states of the LED diminishes. 

% conclusions
The particular solar cell, we use for the \ulp receiver \tv{which one is that and why did we choose it?}, can support a maximum bitrate of 80 $mV$, as the $V_{pp}$ difference becomes close to 10 $mV$. This is the minimum difference in voltage needed by the thresholding circuit to operate.

\begin{figure}[!tb]
\centering
  \includegraphics[width=0.4\textwidth]{solarcellbitrate.pdf}
        \vspace{-4mm}

  \caption{ Solar cell evaluation. \capt{ The ability to distinguish between the ON and OFF states of the bulb becomes difficult at higher bitrates. The particular behaviour is shown by all the solar cells we tested.} }
  \label{solarcellbitrate}
      \vspace{-4mm}

\end{figure}

